\~{O}ptimal Dual Vertex Failure Connectivity Labels

In this paper we present succinct labeling schemes for supporting connectivity queries under vertex faults. For a given $n$-vertex graph $G$, an $f$-VFT (resp., EFT) connectivity labeling scheme is a distributed data structure that assigns each of the graph edges and vertices a short label, such that given the labels of a vertex pair $u$ and $v$, and the labels of at most $f$ failing vertices (resp., edges) $F$, one can determine if $u$ and $v$ are connected in $G \setminus F$. The primary complexity measure is the length of the individual labels. Since their introduction by [Courcelle, Twigg, STACS '07], FT labeling schemes have been devised only for a limited collection of graph families. A recent work [Dory and Parter, PODC 2021] provided EFT labeling schemes for general graphs under edge failures, leaving the vertex failure case fairly open. We provide the first sublinear $f$-VFT labeling schemes for $f \geq 2$ for any $n$-vertex graph. Our key result is $2$-VFT connectivity labels with $O(\log^3 n)$ bits. Our constructions are based on analyzing the structure of dual failure replacement paths on top of the well-known heavy-light tree decomposition technique of [Sleator and Tarjan, STOC 1981]. We also provide $f$-VFT labels with sub-linear length (in $|V|$) for any $f=o(\log\log n)$, that are based on a reduction to the existing EFT labels.

==> additional-related-work.tex <==
\section{Additional Related Work}\label{sec:add-work}
Our dual-failure vertex connectivity labels are also closely related to \emph{connectivity sensitivity oracles} \cite{DuanConnectivitySODA17,DuanP20}, that provide low-space centralized data-structure for supporting connectivity queries in presence of vertex faults. The main goal in our setting in providing a \emph{distributed} variant of such construction, where each vertex holds only $S(n)/n$ bits of information, where $S(n)$ is the global space of the centralized data-structure. For dual failures, data structures based SPQR trees \cite{BattistaT89} use optimal space of $O(n)$ and report connectivity queries in constant time \cite{BattistaT96}. Duan and Pettie \cite{DuanConnectivitySODA17,DuanP20} provided an ingenues construction that supports multiple vertex faults in nearly optimal space of $\widetilde{O}(n)$. These constructions are built upon highly centralized building blocks, and their distributed implementation is fairly open.

Another seemingly close variant of FT connectivity labels has been studied by Katz, Katz, Korman and Peleg \cite{KatzKKP04}. They provide a labeling scheme, for a given integer $k$, that allows one to report $\min\{k, \kappa(u,v)\}$, where $\kappa(u,v)$ is the vertex-connectivity of a given query pair $u$ and $v$. The state-of-the-art label length for this setting is $O(k \log n)$, due to Hsu and Lu \cite{HsuL09}, which is also tight by \cite{KatzKKP04}. In a very recent work \cite{PettieSTOC22} presented an optimal construction of $k$-vertex connectivity oracles w.r.t space and query time. FT connectivity labels differ from this above mentioned setting.  In our setting, we are also given the labels of the faults $F$, and it is required to determine $u$-$v$ connectivity in $G \setminus F$. This is in particular challenging in cases where a removal of a single vertex disconnects $u$ and $v$, i.e., $\kappa(u,v)=1$. In the latter case, our decoding algorithm is required to return distinct answers for distinct set of faults.

==> sublinear-labels.tex <==
\section{Sublinear $f$-VFT Labels}\label{sec:sublinear}

In this section, we provide an $f$-VFT labeling scheme with sublinear size for any $f=o(\log\log n)$. Note that labels of near-linear size are directly obtained by the $f$-EFT labeling scheme of \cite{DoryP21} (e.g., by including in the labels of a vertex, the EFT-labels of all its incident edges). We show:

\begin{theorem}[$f$-VFT Labels with Sublinear Size]\label{thm:sublinear-labels}
For every $n$-vertex graph $G=(V,E)$ and fixed parameter $f=o(\log\log n)$, there is a polynomial time randomized algorithm for computing $f$-VFT labels of size $O(n^{1-1/2^{f-1}}\cdot \log^{3f}n)$. For every query $\langle u,v, F \rangle$ for $F \subseteq V$, $|F|\leq f$, the correctness holds w.h.p.
\end{theorem} 

We use the following EFT-labeling scheme of Dory and Parter \cite{DoryP21}, whose label size is independent in the number of faults. The correctness guarantee holds w.h.p. for a \emph{polynomial} number of queries. 
\begin{theorem}[Slight Restatement of Theorem 3.7 in \cite{DoryP21}]\label{thm:EFT-labels}
For every undirected $n$-vertex graph $G=(V,E)$, there is a randomized EFT connectivity labels $\EFTLabel: V \cup E \to \{0,1\}^{\ell}$ of length $\ell=O(\log^3 n)$ bits (independent in the number of faults).
For a given triplet along w the $\EFTLabel$ labels of $u,v \in V$ and every edge $F \subseteq E$, the decoding algorithm determines, w.h.p., if $u$ and $v$ are connected in $G \setminus F$. 
\end{theorem}

\paragraph{The Labels.} Our starting observation is that one can assume, w.l.o.g., that $|E(G)|\leq fn$ edges. This holds as it is always sufficient to apply the labeling scheme on the sparse $f$ (vertex) connectivity certificate of $G$, which has at most $f n$ edges, see e.g., \cite{cheriyan1993scan}. The labeling scheme is inductive where the construction of $f$-VFT labels is based on the construction of $(f-1)$ VFT labels given by the induction assumption. For the base of the induction ($f=1$), we use the $1$-VFT labels of Theorem \ref{thm:Single-fault-labels}. The approach is then based on dividing the vertices into high-degree and low-degree vertices based on a degree threshold $\Delta=\widetilde{O}(n^{1-1/2^{f-1}})$. Formally, let $V_H$ be all vertices with degree at least $\Delta$. 
By our assumption, the number of high-degree vertices is at most $|V_H|\leq O(f n/ \Delta)$. Letting $\EFTLabel(\cdot)$ denote that $f$-EFT labeling scheme of Theorem \ref{thm:EFT-labels} by \cite{DoryP21}, the $f$-VFT label of $v$, denoted as $\VFTLabel{f}(v)$, is given by:

\begin{framed}
	\noindent\textbf{Label $\VFTLabel{f} (v)$ of $v \in V$:}
	\begin{itemize}
	  \item $\EFTLabel{f}(v)$
		\item $\VFTLabel{f-1}(v,G \setminus \{x\})$ for every $x \in V_H$
		\item For $v \in V \setminus V_H$: $\EFTLabel(e=(u,v))$ for every $(u,v) \in G$.
	\end{itemize}
\end{framed}

\paragraph{The Decoding Algorithm.} Consider a query $\langle u,v, F \rangle \in V \times V \times V^{\leq f}$. We distinguish between two cases, based on the degrees of the faults $F$ in the graph $G$. Assume first that there exists at least one high-degree vertex $x \in F \cap V_H$,. In this case, the labels of $\{u,v\}$ and every $y \in F \setminus \{x\}$, includes the $\VFTLabel{f-1}(v,G \setminus \{x\})$. We can then determine the $F$-connectivity of $u$,$v$ using the decoding algorithm of the $(f-1)$-VFT labels.
It remains to consider the case where all vertices have low-degrees. In this case, we have the EFT labels of $u,v$, and all failed edges, incident to the failed vertices. This holds as the label of every failed vertex $x \in F$ contains the 
$\EFTLabel(e=(x,z))$ for each of its incident edges $(x,z)$ in $G$. This allows apply decoding algorithm of Theorem \ref{thm:sublinear-labels} in a black-box manner. 

\paragraph{Label Size.}
We now turn to bound the label size. For every $f \leq n$, let $\sigma_V(f, n), \sigma_E(n)$ be an upper bound on $f$-VFT (resp., EFT) labels for $n$-vertex graphs. Note that by Theorem \ref{thm:sublinear-labels}, $\sigma_E(n)=O(\log^3 n)$ regardless of the number of faults $f$.  Our construction satisfies the following inductive relations:

$$\sigma_V(f, n) \leq \sigma_V(f-1, n-1) \cdot (2nf/\Delta(f,n)) + \Delta(f,n)\cdot \sigma_E(f, n)~,$$

where $\Delta(f,n)$ is the degree threshold $\Delta$ used in the construction of the $f$-VFT labels for $n$-vertex graphs. 
The claim follows by plugging $\Delta(f,n)=\Theta(n^{1-1/2^{f-1}})$, $\sigma_E(n)=O(\log^3 n)$ (from \cite{DoryP21}) and $\sigma_V(f-1, n)=O(\log^2 n)$ by Theorem \ref{thm:Single-fault-labels}. 




%
%
%\paragraph{Tool: Fault-Tolerant Sketching.} Our construction is based on computing for each vertex $v$ its sketch information in a family of $K=\Theta(f^2 \log n)$ subgraphs $\mathcal{G}_f=\{G_1,\ldots, G_K\}$. Each subgraph $G_i \in \mathcal{G}_f$ is defined by sampling each vertex $v \in V$ independently with probability of $1/f$. The sugraph $G_i$ is then given by the induced graph $G$ on the sampled vertices. Formally, $G_i=G[V[p]]$ where $V[p] \subseteq V$ is a random sample of vertices obtained by sampling each vertex with probability of $p=1/f$. 
%For every vertex $v$, we then compute a bundle of sketches:
%$$\Sketch_{\mathcal{G}_f}(v)=\{\Sketch_{G_i}(v) ~\mid~ G_i \in \mathcal{G}_f\}.$$
%Our $f$-VFT labels are based on the construction of $f$-EVT labels by \cite{DoryP21} which we will use in an almost black-box manner, with the only distinction that we use the FT-sketch information, e.g., $\Sketch_{\mathcal{G}_f}(v)$ instead of 
%$\Sketch_{\mathcal{G}}(v)$. The useful property of these sketches is summarized in the following lemma:
%
%\begin{lemma}\label{lem:useful-FT-sketch}
%Fix $F \subseteq V$ where $|F|\leq f$ and consider a subset $C$ of vertices such that (i) $C \cap F=\emptyset$, (ii) $G[C]$ is connected and (iii) $C$ is not a maximal connected component in $G \setminus F$. 
%Then, given $\Sketch_{\mathcal{G}_f}(C)$, one can determine a $G$-outgoing edge $(u,v) \in C \times (V \setminus C)$ such that $v \notin F$, with high probability.
%\end{lemma}
%\begin{proof}
%Let $E_F(C)=\{ (u,v) \in G \setminus F ~\mid~ u \in C, v \notin C\}$. Since $C$ is not a maximal connected component in $G \setminus F$, we have that $E_F(C)$ is nonempty. By the properties of the linear sketches, it is sufficient to show that w.h.p., there exists a subgraph $G_i \in \mathcal{G}_f$ satisfying that 
%\begin{equation}\label{eq:hit-miss-Gi}
%F \cap V(G_i) = \emptyset \mbox{~~and~~} E_F(C) \cap E(G_i) \neq \emptyset~.
%\end{equation}
%Consider a fixed edge $(u,v) \in E_F(C)$. The probability that $u,v \in V(G_i)$ and $F \cap V(G_i)=\emptyset$ is equal to $p^2 \cdot (1-p)^f =\Theta(1/f^2)$. Since $\mathcal{G}_f$ contains $\Theta(f^3 \log n)$ independent subgraphs, with probability of $1-1/n^{cf}$, there exists at least one subgraph $G_i \in \mathcal{G}_f$ that satisfies Eq. (\ref{eq:hit-miss-Gi}), the claim follows.  
%\end{proof}
%
%In the EFT-labeling scheme of \cite{DoryP21}, the decoding algorithm is based on computing the $G$-sketch of each component in $T \setminus F$ for a faulty edge set $F$. This sketch information was then updated to sketch in $G \setminus F$ simply by canceling the edges $F$ from their corresponding entries in the sketch information. In our context, the decoding algorithm will receive the edge labels of only the tree-edges incident to the failed vertices. This will prevent us from employing this type of cancellation. The lack of edge labels is compensated by including the FT-sketches, which provides a sufficient amount of redundant sketch information in multiple subgraphs to avoid the faulty vertices. 
%
%
%\paragraph{The Labels.}
%The construction is inductive, where the computation of $f$-VFT labels for every $f \geq 2$ is based on $(f-1)$-VFT labels of size $\widetilde{O}(n^{1-1/2^{f-2}})$. The base of this induction for $f=1$ is given by the $1$-VFT labels of Theorem \ref{thm:Single-fault-labels}. Assume now that for every $g \in \{1,\ldots, f-1\}$ there are labels of size 
%$\sigma(g,n)=c \cdot n^{1-1/2^{g-1}}\cdot \log^{3g} n$ for some constant $c$. We now describe the construction of the $f$-VFT labels.
%
%Let $T$ be a spanning tree in $G$. We define a degree threshold $\Delta$ and denote a vertex $v$ to be \emph{high-degree} if $\deg(v,T)\geq \Delta$, and \emph{light-degree} otherwise. Let $V_H$ denote the set of high-degree vertices in $T$. 
%Let $EL_{f}$ denote the $f$-EFT labels of \cite{DoryP21} with the only modification that we use the FT-sketch information, rather than the $G$-sketch information. In addition, let $VL_{f-1,G'}$ denote the $(f-1)$-VFT labels for a subgraph $G'$ (as given by the induction assumption). The $f$-VFT label of vertex $v$ contains the labels $VL_{f-1,G\setminus \{x\}}(v)$ for every $x \in V_H$, and $EL_{f,G}(v)$. For a low-degree vertex $v$, the label contain, in addition, also the edge labels $EL_{f,G}(e)$ for each of its incident edges $e$ in $T$. 
%
%\paragraph{Label Size.} The label $VL_{f,G}(v)$ contains $|V_H|$ sublabels $VL_{f-1,G\setminus \{x\}}(v)$ for every $x \in V_H$. Since $|V_H|\leq 2n/\Delta$, this consumes at most $2\sigma_{f-1,n} \cdot n/\Delta$ bits. In addition, each sketch $EL_{f,G}(e)$ has size $c' \cdot f^3 \log^4 n$. Altogether, the label size is bounded by
%$\sigma(f,n) \leq \sigma(f-1,n) \cdot (2n/\Delta)+c' \cdot f^3 \log^4 n \cdot \Delta \leq c \cdot n^{1-1/2^{f-1}}\cdot \log^{3f} n~,$ where the last inequality follows by setting $\Delta=\Theta(n^{1-1/2^{f-1}}/(f^{1.5}\log^2 n)$. 
%
%
%\paragraph{The Decoding.} Consider a triplet $\langle u,v, F \rangle$ for $F \subseteq V$ and $|F|\leq f$. 
%The decoding procedure is divided into two cases. For the first case assume that there exists some vertex $x \in F \cap V_H$. In this case, the labels of all the vertices $u,v, F \setminus \{x\}$ contains the $(f-1)$-VFT labels in the graph $G \setminus \{x\}$, which can be used to determine the $u$-$v$ connectivity in $(G \setminus \{x\})\setminus (F \setminus \{x\})$, as $|F \setminus \{x\}|\leq f-1$. 
%
%It remains to consider the case where all vertices in $F$ are low-degree. We then have the following collection of labels 
%$\{EL_{f,G}(w), w \in \{u,v\} \cup F\}$ and the labels $EL_{f,G}(e)$ for every edge $e$ incident to $F$ in $T$. This allows us to obtain the FT-sketches of each component in $T \setminus F$. Specifically, for every component $C \in T \setminus F$, we have $\Sketch_{\mathcal{G}_f}(C)$. Using this information, the decoding algorithm simulates $O(\log n)$ phases of the Bor\r{u}vka algorithm in $G \setminus F$. 
%
%This simulation as $O(\log n)$ phases. In each phase $i$, we are given the current components $\mathcal{C}_i$ in $G \setminus F$ along with $\Sketch_{\mathcal{G}_f}(C)$ for every $C \in \mathcal{C}_i$. The goal of this phase is to compute, with constant probability, an outgoing edge for each component  $C \in \mathcal{C}_i$ that is still growable in $G \setminus F$. This holds by the properties of the FT-sketches in Lemma \ref{lem:useful-FT-sketch}. 
%\textbf{MP: I still need to write more formally, unready for pass yet.}
%




